Empirical Policy Evaluation with Supergraphs

We devise and analyze algorithms for the empirical policy evaluation problem in reinforcement learning. Our algorithms explore backward from high-cost states to find high-value ones, in contrast to forward approaches that work forward from all states. While several papers have demonstrated the utility of backward exploration empirically, we conduct rigorous analyses which show that our algorithms can reduce average-case sample complexity from $O(S \log S)$ to as low as $O(\log S)$.

==> prelim.tex <==
%\section{Background on PageRank} \label{secPrelim}

%\subsection{PageRank contributions and policy evaluation} \label{secPageRankPolicy}

%Before describing the relevant PageRank estimators, we discuss PageRank and its connection to policy evaluation. Given discount factor $\alpha$ and transition matrix $Q$, %(typically the row-normalized adjacency matrix of some underlying graph), 
%the \textit{PageRank vector} $\mu$ is the stationary distribution of the Markov chain with transition matrix $(1-\alpha) 1_{S \times S} / S + \alpha Q$. Note this transition matrix is irreducible and aperiodic, so $\mu$ exists and is unique. Also, viewing $\mu$ as a row vector, we observe
%\begin{equation}\label{eqPrClosedForm}
%\mu = \mu \left( \frac{ (1-\alpha) 1_{S \times S} }{ S } + \alpha Q \right) = \frac{ (1-\alpha) 1_{1 \times S} }{ S } + \alpha \mu Q \quad \Rightarrow \quad \mu = \frac{(1-\alpha) 1_{1 \times S}}{S} (I-\alpha Q)^{-1}  ,
%\end{equation}
%where $\mu 1_{S \times S} = 1_{1 \times S}$ assuming $\mu$ is normalized to sum to $1$. In the PageRank literature, $Q$ is typically the row-normalized adjacency matrix of some graph, and $\mu$ is interpreted as a centrality measure for the nodes of the graph; this interpretation has been exploited in many graph mining applications \cite{gleich2015pagerank}.
%
%PageRank offers a natural generalization called \textit{Personalized PageRank} (PPR). Given $s \in \mathcal{S}$, the \textit{PPR vector} corresponding to $s$ is defined as the stationary distribution $\mu_s$ corresponding to $(1-\alpha) 1_{S \times 1} e_s^{\tr} + \alpha Q$. Note that by the same logic of \eqref{eqPrClosedForm}, $\mu_s = (1-\alpha) e_s^{\tr} (I - \alpha Q)^{-1}$. Thus, combined with \eqref{eqPrClosedForm},
%\begin{equation}\label{eqPrPprAvg}
%\mu = (1-\alpha) \frac{1_{1 \times S}}{S} (I-\alpha Q)^{-1} = (1-\alpha) \frac{\sum_{s=1}^S e_s}{S} (I-\alpha Q)^{-1}  = \frac{1}{S} \sum_{s=1}^S \mu_s , 
%\end{equation}
%i.e.\ the PageRank vector is simply the average of the PPR vectors. Similar to PageRank, PPR is interpreted as a centrality measure from the perspective of node $s$ and has many application; again, see \cite{gleich2015pagerank}.
%
%From this discussion, we describe the \textit{PageRank contributions} problem. First, for $s^* \in \mathcal{S}$, \eqref{eqPrPprAvg} implies the PageRank value $\mu(s^*)$ is the average of the PPR values $\{ \mu_s(s^*) \}_{s=1}^S$. Viewing this set as a vector, we have $\{ \mu_s(s^*) \}_{s=1}^S = (1-\alpha) (I - \alpha Q)^{-1} e_{s^*}$. The PageRank contributions problem is to estimate this vector: given $s^*$, one aims to find which PPR values $\mu_s(s^*)$ contribute the most to the average of these values, i.e.\ to the PageRank $\mu(s^*)$. Historically, this problem arose owing to the issue of link spam on the web \cite{andersen2008local}. For our purposes, the key observation is that $ (1-\alpha) (I - \alpha Q)^{-1} e_{s^*}$ is  the value function \eqref{eqValFunc} in the case $c = e_{s^*}$. Thus, our algorithms will be based on PageRank contribution estimators, namely, the algorithm from \cite{andersen2008local}.

brief PPR defintion

\subsection{Estimators for PageRank contributions} \label{secPageRankAlgs}

\subsubsection{The \texttt{Approx-Contributions} algorithm} \label{secPageRankAlgsAC}

The algorithm from \cite{andersen2008local} is (unsurprisingly) called \texttt{Approx-Contributions} and is defined in Algorithm \ref{algApproxCont}. As mentioned in Section \ref{secPageRankPolicy}, the algorithm restricts to the case $c = e_{s^*}$, but here we describe the algorithm for general $c \in \R_+^S$ as this requires no additional work. The algorithm takes as input transition matrix $Q$ (assumed to be known in \cite{andersen2008local}), cost vector $c$, discount factor $\alpha$, and desired accuracy $\epsilon$, and initializes \textit{estimate vector} $\hat{v}_0 = 0_{S \times 1}$ and \textit{residual vector} $r_0 = c$. The estimate and residual vectors are then iteratively updated so as to estimate $v$. Conceptually, the iterative update is similar to the power iteration discussed in Section \ref{secIntroMotivation}. However, here each iteration explores the incoming neighbors of a \textit{single high-residual state}, rather than exploring the incoming neighbors of \textit{potentially many states} as in Section \ref{secIntroMotivation}. More precisely, the $k$-th iterative update samples a state $s_k$ uniformly from $\argmax_{s \in \mathcal{S}} r_{k-1}(s)$ (Line \ref{algApproxCont_sampleSk} of Algorithm \ref{algApproxCont}) and pushes residual mass from $s_k$ to other states (Lines \ref{algApproxCont_skUpdate}-\ref{algApproxCont_sUpdate}). The precise form of this push operation ensures
\begin{equation}\label{eqInvariantKnownQ}
\hat{v}_k(s) + \mu_s r_k = v(s)\ \forall\ k \in \{0,1,\ldots\} , s \in \mathcal{S} .
\end{equation}
This continues until the first iteration $k$ for which $\| r_k \|_{\infty} \leq \epsilon$. Letting $k_* = \min \{ k \in \Z_+ : \| r_k \|_{\infty} \leq \epsilon \}$ denote this iteration, \eqref{eqInvariantKnownQ} ensures that $\hat{v}_{k_*}(s)$ is an $\epsilon$-accurate estimate of $v(s)$, since
\begin{equation}\label{eqInvariantKnownQKstar}
| \hat{v}_{k_*}(s) - v(s) | \leq \sum_{s'=1}^S \mu_s(s') r_{k_*}(s') \leq \epsilon \sum_{s'=1}^S \mu_s(s') = \epsilon .
\end{equation}
Thus, the fact that \texttt{Approx-Contributions} produces an accurate estimate relies fundamentally on \eqref{eqInvariantKnownQ}. Note $v(s) = \mu_s c$ and thus \eqref{eqInvariantKnownQ} is a fixed-point equation (in $\mu_s$); this is precisely the fixed-point equation mentioned in Section \ref{secIntroOverview}. Owing to the fact that \eqref{eqInvariantKnownQ} is preserved across iterations $k$, it is referred to as the \textit{invariant}. For a proof of the invariant, see \cite[Lemma 1]{andersen2008local}; we also discuss this proof in Remark \ref{remInvariantProofKnownQ} below.

\begin{algorithm}
\caption{\texttt{Approx-Contributions} (from \cite{andersen2008local})} \label{algApproxCont}
\KwIn{Transition matrix $Q$; cost vector $c$; discount factor $\alpha$; termination parameter $\epsilon$}
$k = 0$, $\hat{v}_k = 0_{S \times 1}$, $r_k = c$ \label{algApproxContInit} \\
\While{$\|r_k\|_{\infty} > \epsilon$}{%
	$k \leftarrow k+1$, $s_k \sim \argmax_{s \in \mathcal{S}} r_{k-1}(s)$ uniformly \label{algApproxCont_sampleSk} \\
	\For{$s \in \mathcal{S}$}{
		\lIf{$s = s_k$}{$\hat{v}_k(s) = \hat{v}_{k-1}(s) + (1-\alpha) r_{k-1}(s)$, $r_k(s) = \alpha Q(s,s_k) r_{k-1}(s_k)$} \label{algApproxCont_skUpdate}
		%\lElseIf{$s \neq s_k, Q(s,s_k) > 0$}{$\hat{v}_k(s) = \hat{v}_{k-1}(s)$, $r_k(s) = r_{k-1}(s) + \alpha Q(s,s_k) r_{k-1}(s_k)$}
		%\lElse{$\hat{v}_k(s) = \hat{v}_{k-1}(s)$, $r_k(s) = r_{k-1}(s)$} \label{algApproxCont_sUpdate}
		\lElse{$\hat{v}_k(s) = \hat{v}_{k-1}(s)$, $r_k(s) = r_{k-1}(s) + \alpha Q(s,s_k) r_{k-1}(s_k)$} \label{algApproxCont_sUpdate}
	}
} 
\KwOut{Estimate $\hat{v}_{k}$ of $v = (1-\alpha) \sum_{t=0}^{\infty} \alpha^t Q^t c$}
\end{algorithm}

Note that in \texttt{Approx-Contributions}, we simply discard the $\epsilon$-bounded residual at conclusion of the algorithm; see \eqref{eqInvariantKnownQKstar}. The key idea of the aforementioned bidirectional PageRank estimator from \cite{lofgren2016personalized} is that this residual can be estimated. Indeed, the residual vector is $\{ \mu_s r_{k_*} \}_{s \in \mathcal{S}} = (1-\alpha) ( I - \alpha Q )^{-1} r_{k_*}$, which is precisely the form of the value function \eqref{eqValFunc}. Hence, after running \texttt{Approx-Contributions}, one can use forward exploration techniques to estimate this vector and improve the estimate of $v$. As alluded to in Section \ref{secIntroOverview}, this is the inspiration for our second algorithm, \texttt{Bidirectional-EPE}. Unlike \texttt{Approx-Contributions}, however, the forward exploration stage of the bidirectional PageRank algorithm readily adapts to the case where $Q$ is unknown, so we do not discuss it further here; see Section \ref{secBidirectionalAlgo} for details.




